The onset time of Fermi's golden rule

Fermi's golden rule describes the decay dynamics of unstable quantum systems coupled to a reservoir, and predicts a linear decay in time. Although it arises at relatively short times, the Fermi regime does not take hold in the earliest stages of the quantum dynamics. The standard criterion in the literature for the onset time of the Fermi regime is $t_F\sim1/\Delta\omega$, with $\Delta\omega$ the frequency interval around the resonant transition frequency $\omega_0$ of the system, over which the coupling to the reservoir does not vary appreciably. In this work, this criterion is shown to be inappropriate in general for broadband reservoirs, where the reservoir coupling spectrum takes the form $R\left(\omega\right)\propto\omega^\eta$, and for which it is found that for $\eta>1$, the onset time of the Fermi regime is given by $t_F\propto\left(\omega_{\mathrm{X}}/\omega_0\right)^{\eta-1}\times1/\omega_0$ where $\omega_{\mathrm{X}}$ is the high-frequency cutoff of the reservoir. Therefore, the onset of the Fermi regime can take place at times orders of magnitude larger than those predicted by the standard criterion. This phenomenon is shown to be related to the excitation of the off-resonant frequencies of the reservoir at short times. For broadband reservoirs with $\eta\leq1$, and for narrowband reservoirs, it is shown that the standard criterion is correct. Our findings revisit the conditions of applicability of Fermi's golden rule and improve our understanding of the dynamics of unstable quantum systems.

==> FermiGR_Books <==
MESSIAH

Transitions to an interval of width \epsilon (sufficiently small so that density of states and form factor can be taken out of integral).
"We also suppose t sufficiently large for \epsilon to be much greater than the period of oscillation of the function F_t, that is \epsilon\gg2\pi\hbar/t."
This last inequality is the validity condition of Fermi's golden rule.


COHEN-TANNOUDJI DIU LALOË (p. 1300)

"If t is sufficiently large, F_t can be approximated (within a constant factor) by the Dirac delta function.
[The other quantities in the integral] vary mich more slowly with E. We shall assume here that t is sufficiently large for the variation of the form factor and the density of states over an energy interval of width 4\pi\hbar/t centered at E=E_{\mathrm{i}} to be negligible. We can then replace F_t by its limit."

BASDEVANT DALIBARD

"The time t must be long enough that the frequency width (1/t) of F_t be much smaller than the typical scale of variation of (densité d'états * facteur de forme)."

LE BELLAC

Condition de validité de la règle d'or :
"Si \Delta E est l'intervalle caractéristique de variation de (densité d'états * facteur de forme), alors \hbar/\Delta E doit être petit par rapport à t."

DIRAC

(Not much)

FEYNMAN

(Nothing)

LANDAU LIFSHITZ

"For large t": distributional limit.

BRANSDEN JOACHAIN

"It is often necessary to deal with transitions to a group of final states whose energy lies with a given interval E_{\mathrm{f}}\pm\eta centred about the energy of the final state.
"Assuming that \eta is small enough so that the form factor and the density of states are nearly constant within the integration range, [we take these two out of the integral]. We shall also assume that t is large enough so that \eta satisfies the condition _eta\gg2\pi\hbar/t. Now it is clear that the integral will be small except for transitions which conserve energy."

GRIFFITHS

"Ordinarily, F_t is sharply peaked about the transition frequency whereas the the form factor and the density of states are relatively broad, in that case we may as well replace them by their values at the transition frequency and take them outside the integral."

SCHIFF

"Since the form factor and the density of states are slowly varying and most of the contribution to the integral comes from a narrow range of energy about E_k=E_m, they can be taken outside of the integral."

SAKURAI

"As t\rightarrow\infinity we can take advantage of the distributional limit"

LIBOFF

"Owing to the rapid decay of the square cardinal since function only a slight error is introduced if we integrate over the whole real axis. Furthermore, if we assume that the form factor and the density of states are slowly varying functions of the energy, they may be taken outside the integral."


SMALL INTERVAL OF FINAL STATES:              1
LARGE TIME LIMIT (WIDTH OF INTERVAL):        5

